Safe Adaptive Cruise Control with Road Grade Preview and V2V Communication

We present the design of a safe Adaptive Cruise Control (ACC) which uses road grade and lead vehicle motion preview. The ACC controller is designed by using a Model Predictive Control (MPC) framework to optimize comfort, safety, energy-efficiency and speed tracking accuracy. Safety is achieved by computing a robust invariant terminal set. The paper presents a novel approach to compute such set which is less conservative than existing methods. The proposed controller ensures safe inter-vehicle spacing at all times despite changes in the road grade and uncertainty in the predicted motion of the lead vehicle. Simulation results compare the proposed controller with a controller that does not incorporate prior grade knowledge on two scenarios including car-following and autonomous intersection crossing. The results demonstrate the effectiveness of the proposed control algorithm.

==> Sec_ACC.tex <==
\section{Adaptive Cruise Control}
\label{secACC}


\subsection{Problem Statement and MPC Formulation}
In this study, the controller is designed to operate in two modes, reference tracking mode and target vehicle following mode. 
The reference tracking mode will remain activated as long as the sensors have not yet detected any vehicle ahead. 
In this mode the controller tracks a position-dependent optimal reference velocity profile which has been calculated formerly for a specific route, while incorporating the prior knowledge of grade.


The proposed controller is formulated as a constrained finite horizon optimization problem
\begin{equation}\label{eq:1a}
    \min\limits_{u(.|t)} J = \sum_{k=t}^{t+N}||v(k|t)-v_{Ref}||+\sum_{k=t}^{t+N-1}||u(k|t)||
\end{equation}
\begin{equation}\label{eq:2a}
    \textrm{subject to:} \quad
    x(k+1|t) = f(x(k|t),u(k|t),v_{Ref}(k|t))
\end{equation}
\begin{equation}\label{eq:3a}
v_{min} \leq v(k|t) \leq v_{max}
\end{equation}
\begin{equation}\label{eq:3a}
u_{min} \leq u(k|t) \leq u_{max}
\end{equation}

where $x(k|t)=[s(k|t) \quad v(k|t)]^T$ and $u(k|t)$ are the state variable and control input at time k predicted at time t, respectively, $f$ represents the dynamics and $v_{Ref}$ denotes the target vehicle speed trajectory.  
terminal cost
terminal constraint

Once the sensors detect a vehicle ahead, the controller switches to target vehicle following mode in which the vehicle maintains a safe distance relative to the target vehicle and starts tracking the front vehicle velocity.

\begin{equation*}
    \min\limits_{u(.|t)} J = \sum_{k=t}^{t+N}||v(k|t)-v_{Ref}||+\sum_{k=t}^{t+N-1}||u(k|t)||
\end{equation*}
\begin{equation*}
    \textrm{s.t.} \quad
    x(k+1|t) = f(x(k|t),u(k|t),v_{Ref}(k|t))
\end{equation*}
\begin{equation*}
v_{min} \leq v(k|t) \leq v_{max}
\end{equation*}
\begin{equation*}
u_{min} \leq u(k|t) \leq u_{max}
\end{equation*}
\begin{equation*}
d_{safe} \leq s_{lead}(k|t) - s(k|t) 
\end{equation*}

